RadTimeline: Timeline Summarization for Longitudinal Radiological Lung Findings

Tracking findings in longitudinal radiology reports is crucial for accurately identifying disease progression, and the time-consuming process would benefit from automatic summarization. This work introduces a structured summarization task, where we frame longitudinal report summarization as a timeline generation task, with dated findings organized in columns and temporally related findings grouped in rows. This structured summarization format enables straightforward comparison of findings across time and facilitates fact-checking against the associated reports. The timeline is generated using a 3-step LLM process of extracting findings, generating group names, and using the names to group the findings. To evaluate such systems, we create RadTimeline, a timeline dataset focused on tracking lung-related radiologic findings in chest-related imaging reports. Experiments on RadTimeline show tradeoffs of different-sized LLMs and prompting strategies. Our results highlight that group name generation as an intermediate step is critical for effective finding grouping. The best configuration has some irrelevant findings but very good recall, and grouping performance is comparable to human annotators.

==> sections/literature_review_sections/EHRTemporal.tex <==
% how they represent temporal informatino
\subsection{Understanding Longitudinal EHRs }

%[CURRENT WORK WHAT they do]
 Temporal cues in individual imaging reports describe the evolution of findings when comparing with prior images, which are critical information for radiology report understanding and generation. These NLP systems  \citep{RadGraph2DiseaeseProgression, ClassificationPulmonaryNodularFindingChange, characterizationOfChangeAndSignificanceClinicalFindings} leverage those textual cues to classify findings into change types (e.g. improved, unchanged, etc). Vision language modeling approaches \citep{LearningToExploitTemporalStructureVision, ContrastiveMultiViewLongitudinalXrayGeneratino, wang2024hergen, zhu2023utilizingXrayPrefill}  incorporate longitudinal radiology images as inputs to generate current radiology reports containing temporal information.
 Instead of presenting the comparison results as temporal cues such as "slightly improved", our work aims to enable easy comparison by  displaying lung finding details across longitudinal reports in temporal-related groups. 


%How they summarize  longitudinal EHRs?

Timelines can group related facts from scattered notes for easier tracking and comparison.  To reduce cognitive overload in reading longitudinal notes, HARVEST \citep{Hirsch2015HARVEST} built an interactive visualizer to filter EHR notes on normalized medical problem concepts from a terminology, and physicians report high subjective satisfaction with this tool. Instead of relying on predefined concepts, radiological finding groups can naturally emerge from the notes using coreference relations of the findings.  
\citet{crossDocCorefLongitudinalTrackingRad} present a dataset tracking radiological findings and medical devices across each patient’s reports. They further fine-tune a supervised BERT classifier to predict pairwise coreference between mentions and then merge positive pairs into clusters. However, the supervised approach underperforms the string-matching baseline, indicating the need for further model development.
\citet{Mathai2025PrivacyLLMFindingMatch}  study the finding matching task between two reports, a prior and a follow up report of the same modality, MRI or CT. They use a zero-shot LLM to match a sentence from a follow-up to the sentence that best described the same finding  in the  prior report, reaching moderate agreement with expert references.        

We build an end-to-end longitudinal summarization system to convert a patient’s  longitudinal chest-related radiology reports (CT, X-ray) into a timeline table, leveraing off-the-shelf LLMs and textual representations instead of supervised labels. We first extract atomized lung-finding facts from the raw reports,  then group temporally related facts to display the finding trajectories. This system can extract finding facts with a low incorrect rate ( 3\% ??) on lung findings under human evaluation, and clustering finding facts with near-human performance. 






==> sections/literature_review_sections/long_contexts.tex <==

\subsection{Long Context Challenges for LLMs}

\citet{zeroshotLongClinicalTextSummarizationTemporalReasoning} report  LLMs are struggling in using long clinical contexts in EHRShot disease prediction tasks. Llama 2  with shorter 4K context length  degrades with longer inputs, llama 3 (8K context) is stable, and  Qwen (128K context) shows only a slight positive correlation with longer inputs.  

% How they represent / understand longitudinal EHRs for downstreamt ask? 


LLMs struggle with lengthy inputs when the key information are in the middle of long contexts 
\citep{Liu2023LostInTheMiddle}. Resolving coreference on lenthy inputs can improve long context QA and summarization \cite{liu2025bridgingContextGapLongContextualCoref}. 


clinicalMamba
MedAlign
